Graph Neural Networks for Graphs with Heterophily: A Survey

Recent years have witnessed fast developments of graph neural networks (GNNs) that have benefited myriad graph analytic tasks and applications. Most GNNs rely on the homophily assumption that nodes belonging to the same class are more likely to be connected. However, as a ubiquitous graph property in numerous real-world scenarios, heterophily, i.e., nodes with different labels tend to be linked, significantly limits the performance of tailor-made homophilic GNNs. Hence, GNNs for heterophilic graphs are gaining increasing research attention to enhance graph learning with heterophily. In this paper, we provide a comprehensive review of GNNs for heterophilic graphs. Specifically, we propose a systematic taxonomy that governs existing heterophilic GNN models, along with general summaries and detailed analyses. Furthermore, we discuss the relationship between heterophily and various graph research domains, aiming to facilitate the development of more effective GNNs across a spectrum of practical applications and learning tasks in the graph research community. In the end, we point out potential directions to advance and inspire future research and applications on heterophilic graph learning with GNNs.

==> 04datasets.tex <==
% 原版
\begin{comment}
\begin{table*}[t!]
\centering
\caption{Statistics of heterophilic datasets. For comparison, the homophily metrics $h_n$ and $h_e$ of Cora dataset are $0.??$ and $0.83$, respectively.}
% \begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{l|ccccccc}
\toprule
\textbf{Dataset} & \textbf{Domain} & \textbf{\#Nodes} & \textbf{\#Edges}  & \textbf{\#Classes} & \textbf{\#Features} & \textbf{$h_n$} & \textbf{$h_e$}\\ \hline
Cornell       & Uni. Web Page      & 183      & 295       & 5       & 1,703     & 0.11  & 0.30\\ 
Texas         & Uni. Web Page      & 183      & 309       & 5       & 1,703     & 0.06  & 0.11\\ 
Wisconsin     & Uni. Web Page      & 251      & 499       & 5       & 1,703     & 0.16  & 0.21\\ 
Chameleon     & Wiki. Web Page     & 2,277    & 36,101    & 5       & 2,325     & 0.25  & 0.23\\ 
Squirrel      & Wiki. Web Page     & 5,201    & 216,933   & 5       & 2,089     & 0.22  & 0.22\\ 
Actor         & Actor Co-Occur.    & 7,600    & 29,926    & 5       & 931       & 0.24  & 0.22\\ 
\hline
Penn94        & Social Network     & 41,554   & 1,362,229 & 2       & 5         & 0.??  & 0.47\\
twitch-gamers & Social Network     & 168,114  & 6,797,557 & 2       & 7         & 0.??  & 0.55\\
arXiv-year    & Citation Network   & 169,343  & 1,166,243 & 5       & 128       & 0.??  & 0.22\\
genius        & Social Network     & 421,961  & 984,979   & 2       & 12        & 0.??  & 0.62\\
pokec         & Social Network     & 1,632,803& 30,622,564& 2       & 65        & 0.??  & 0.45\\
wiki          & Wiki. Web Page     & 1,925,342&303,434,860& 5       & 600       & 0.??  & 0.39\\
snap-patents  & Citation Network   & 2,923,922& 13,975,788& 5       & 269       & 0.??  & 0.07\\
\bottomrule
\end{tabular}
% \end{adjustbox}
\label{tab:dataset}
\end{table*}
\end{comment}
% 1.31 新
% \begin{table*}[t!]
% \centering
% \caption{Statistics of heterophilic datasets. For comparison, the homophily metrics $h_n$ and $h_e$ of Cora dataset are $0.??$ and $0.83$, respectively.}
% % \begin{adjustbox}{width=1\columnwidth,center}
% \begin{tabular}{c|ccccccccccccc}
% \toprule
%  & Cornell & Texas & Wisconsin & Chameleon & Squirrel & Actor & Penn94 & twitch-gamers & arXiv-year & genius & pokec & wiki & snap-patents \\

% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \label{tab:dataset}
% \end{table*}

\begin{comment}
\begin{table*}[t]
\centering
\caption{}
\label{tab:datasets}
\renewcommand\arraystretch{1.3}
\begin{LARGE}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccccc}
\toprule
\multirow{2}{*}{Datasets} & \multicolumn{3}{c}{WebKB Webpage}    & Author Co-occurrence & \multicolumn{3}{c}{Wikipedia Webpage} & \multicolumn{2}{c}{Citation} & \multicolumn{5}{c}{Social Networks}                               & Webpage Review \\
                          & Cornell    & Wisconsin  & Texas      & Actor                & Chameleon  & Squirrel   & Wiki        & Snap-patents   & ArXiv-Year  & Penn94    & Twitch-Gamers & Deezer-Europe & Genius   & Pokec      & YelpChi        \\ \midrule
\# Nodes                  & 183        & 251        & 183        & 7,600                & 2,277      & 5,201      & 1,925,342   & 2,923,922      & 169,343     & 41,554    & 168,114       & 28,281        & 421,961  & 1,632,803  & 45,954         \\
\# Edges                  & 295        & 499        & 309        & 33,544               & 36,101     & 217,073    & 303,434,860 & 13,975,788     & 1,166,243   & 1,362,229 & 6,797,557     & 92,752        & 984,979  & 30,622,564 & 3,846,979      \\
\# Features               & 1,703      & 1,703      & 1,703      & 931                  & 2,325      & 2,089      & 5           & 5              & 5           & 2         & 2             & 31,241        & 2        & 2          & 32             \\
\# Classes                & 5          & 5          & 5          & 5                    & 5          & 5          & 600         & 269            & 128         & 5         & 7             & 2             & 12       & 65         & 2              \\
H\_("edge ")(G)           & 0.5669     & 0.448      & 0.4106     & 0.375                & 0.2795     & 0.2416     & -           & -              & -           & -         & -             & 0.5251        & -        & -          & 0.773          \\
H\_("node ")(G)           & 0.3855     & 0.1498     & 0.0968     & 0.221                & 0.247      & 0.2156     & 0.39        & 0.07           & 0.22        & 0.47      & 0.55          & 0.5299        & 0.62     & 0.45       & 0.7698         \\
Data Splits(\%)           & 60//20//20 & 60//20//20 & 60//20//20 & 60//20//20           & 60//20//20 & 60//20//20 & 50/25/25    & 50/25/25       & 50/25/25    & 50/25/25  & 50/25/25      & 50/25/25      & 50/25/25 & 50/25/25   & 50/25/25      \\\bottomrule
\end{tabular}
}
\end{LARGE}
\end{table*}
\end{comment}

\begin{table*}[t]
\centering
% \renewcommand\arraystretch{1.0}
%\begin{footnotesize}
\caption{Statistics of real-world heterophilic graph benchmarks. }
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{p{3.5cm}p{2.5cm}cccccc}
\toprule
\multicolumn{1}{l}{Types}        & Datasets      & \# Nodes  & \# Edges    & \# Features & \# Classes & $\mathcal{H}_{node}$ & $\mathcal{H}_{edge}$  \\ \midrule
\multirow{3}{*}{WebKB Webpage}     & Cornell       & 183       & 295         & 1,703       & 5          & 0.11          & 0.30        \\
                                   & Texas         & 183       & 309         & 1,703       & 5          & 0.06          & 0.11       \\
                                   & Wisconsin     & 251       & 499         & 1,703       & 5          & 0.16           & 0.21              \\\hline
Author Co-occurrence               & Actor         & 7,600     & 33,544      & 931         & 5          & 0.24           & 0.22           \\\hline
\multirow{3}{*}{Wikipedia Webpage} & Chameleon     & 2,277     & 36,101      & 2,325       & 5          & 0.25          & 0.23       \\
                                   & Squirrel      & 5,201     & 217,073     & 2,089       & 5          & 0.22          & 0.22         \\
                                   & Wiki          & 1,925,342 & 303,434,860 & 600           & 5        & -               & 0.39               \\\hline
\multirow{2}{*}{Citation}          & ArXiv-Year    & 169,343   & 1,166,243   & 128           & 5        & -               & 0.22        \\
                                   & Snap-patents  & 2,923,922 & 13,975,788  & 269           & 5        & -               & 0.07             \\\hline
\multirow{5}{*}{Social Networks}   & Deezer-Europe & 28,281    & 92,752      & 31,241      & 2          & 0.53          & 0.53     \\
                                   & Penn94        & 41,554    & 1,362,229   & 5           & 2          & -               & 0.47            \\
                                   & Twitch-Gamers & 168,114   & 6,797,557   & 7           & 2          & -               & 0.55              \\
                                   & Genius        & 421,961   & 984,979     & 12           & 2         & -               & 0.62                \\
                                   & Pokec         & 1,632,803 & 30,622,564  & 65           & 2         & -               & 0.45               \\\hline
Webpage Review                     & YelpChi       & 45,954    & 3,846,979   & 32          & 2          & 0.77           & 0.77        \\\bottomrule
\end{tabular}
}
\label{tab:datasets}
%\vspace{-2mm}
%\end{footnotesize}
\end{table*}


\begin{comment}
To empirically evaluate the model performance on real-world heterophilic graphs, most of the current works conduct experiments on the benchmarks containing $6$ datasets proposed by \cite{geom_pei2020geom} . Among these datasets, Cornell, Texas, and Wisconsin are three subdatasets from WebKB web page dataset \cite{garcia2016using}, where nodes are the web pages from computer science departments of different universities, and edges are mutual links between pages. Chameleon and Squirrel are two web page datasets collected from Wikipedia \cite{rozemberczki2021multi}, where nodes are web pages on specific topics and edges are hyperlinks between them. Actor is an actor co-occurrence network \cite{tang2009social} where nodes are actors and edges mean two actors are co-occur on the same Wikipedia page. 
Very recently, a series of new benchmark datasets with larger scales and from diverse areas is proposed by \cite{lim2021large}, including four online social network datasets (Penn94, Pokec, genius, and twitch-gamers), two citation network datasets (arXiv-year and snap-patents), and a Wikipedia web page dataset (wiki). 
Table~\ref{tab:dataset} summarizes the statistics of all benchmark datasets. 
\end{comment}

To provide the data support for the development of heterophilic graph learning, we collect and list current real-world benchmarks of heterophilic graph datasets with detailed statistics, as shown in Table~\ref{tab:datasets}.

Most current works conduct experiments for empirical evaluations on the first $6$ datasets in Table~\ref{tab:datasets}, which are originally presented by the work \cite{geom_pei2020geom}. Specifically, Cornell, Texas, and Wisconsin are three subdatasets from WebKB web-page dataset \cite{garcia2016using}, where nodes are the web pages from computer science departments of different universities, and edges are mutual links between pages. Chameleon and Squirrel are two web page datasets collected from Wikipedia \cite{rozemberczki2021multi}, where nodes are web pages on specific topics and edges are hyperlinks between them. Actor is an actor co-occurrence network \cite{tang2009social}, where nodes are actors and edges mean two actors are co-occurred on the same Wikipedia page. 
%Note that, for comprehensively understanding the difference between homophily and heterophily, current works usually evaluate their models on traditional Cora, Pubmed and Citeseer graphs that have strong homophily, further illustrating the generalization ability of their models.

Very recently, a series of new benchmark datasets with larger scales from diverse areas are collected and released by \cite{lim2021large} and~\cite{lim2021new}, including a Wikipedia web page dataset (Wiki), two citation network datasets (ArXiv-year and Snap-Patents), five online social network datasets (Penn94, Pokec, Genius, Deezer-Europe, and Twitch-Gamers), as well as a web-page hotel and restaurant review dataset (YelpChi). It can be anticipated that more publicly available heterophilic benchmarks are built to facilitate and advance the research and applications of GNNs on heterophilic graphs.







==> bio-v2.tex <==
\section*{Biographies}
\begingroup
\footnotesize

\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/xinz.jpg}}]{Xin Zheng} is a Lecturer with the School of Computing Technologies at RMIT University, Australia. She received a Ph.D. degree in computer science from Monash University, Australia, in 2024. 
Her research interests include data-centric graph machine learning and automated graph MLOps. To date, she has published research papers in top-tier journals and conferences, including IJCV, PR, NeurIPS, ICLR, ICML, and Web Conference.
\end{IEEEbiography}
%\vspace{1.2em}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/WangY.eps}}]{Yi Wang} received her Ph.D. degree in Computer Science and Technology from Zhejiang Normal University, Jinhua, China, in 2025. She is presently a postdoctoral fellow at the City University of Hong Kong. She has published several papers in top-tier journals and conferences, inclusing IEEE TCYB, PR, NN, ICML, AAAI, IJCAI. Her research interests include graph neural networks, hypergraph computing, graph data mining, etc.
\end{IEEEbiography}
%\vspace{1.2em}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/Yixin.jpg}}]{Yixin Liu}
is a Lecturer and ARC DECRA Fellow at Griffith University. He received his Ph.D. in Artificial Intelligence (AI) from Monash University, Australia, and his Bachelor’s and Master's degrees from Beihang University, China. His research concentrates on data mining, machine learning, graph analytics, and anomaly detection. To date, he has published more than 30 research papers in top-tier journals and conferences, including IEEE TKDE, IEEE TNNLS, NeurIPS, KDD, AAAI, and Web Conference. He is a recipient of Google Ph.D. Fellowship in 2022.
\end{IEEEbiography}
\vspace{1.5em}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/MingLi.jpg}}]{Ming Li}
received the Ph.D. degree from the Department of Computer Science and Information Technology, La Trobe University, Australia, in 2017. After that, he completed two Postdoctoral Fellowship positions with the Department of Mathematics and Statistics, La Trobe University, Australia, and the Department of Information Technology in Education, South China Normal University, China, respectively. He is currently a `Shuang Long Scholar' Distinguished Professor with Zhejiang Key Laboratory of Intelligent Education Technology and Application, Zhejiang Normal University, China. His research interests include hypergraph/graph neural networks, graph machine learning, hypergraph learning, etc. To date, he has published over 150 research papers in top-tier
journals and conferences, including IEEE TPAMI, Artificial Intelligence, IEEE TKDE, IEEE TNNLS, IEEE TCYB, ICML, AAAI etc. He is an Associate Editor of \emph{Pattern Recognition}, \emph{Neural Networks}, and an Editorial Board Member of \emph{Machine Learning}. He is the recipient of the AAAI 2026 Outstanding Paper Award. 
\end{IEEEbiography}
\vspace{4.5em}
\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/miaoz.jpeg}}]{Miao Zhang}
received the Ph.D. degree from the University of Technology Sydney (UTS), Australia. He is currently a Professor with Harbin Institute of Technology (Shenzhen), Shenzhen, China. Before that, he was an Assistant Professor at Aalborg University, Aalborg, Denmark. His major research interests include AutoML, model compression, and continual learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/dijin.png}}]{Di Jin}
received the Ph.D. degree in computer science from Jilin University, Changchun, China, in 2012. He was a research scholar in DMG at UIUC during 2019 to 2020. He is currently a Full Professor with the College of Intelligence and Computing, Tianjin University, Tianjin, China. His research interests include graph data mining and graph machine learning, especially on community detection, network embedding and GNNs. To date, he has published more than 100 research papers in top-tier journals and conferences, including the TKDE, TNNLS, TYCB, AAAI, IJCAI, ICML, NeurIPS, and WWW. He serves as the Associate Editor of Information Sciences, Action Editor of Neural Networks, PC Board Member of IJCAI 2022-2024, and Senor PCs in IJCAI/AAAI. He was the recipient of the Best Paper Award Runner-Up of WWW 2021, Best Paper Student Paper Runner-Up of ICDM 2021, and Rising Star Award of ACM Tianjin at 2018.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/yup.jpg}}]{Philip S. Yu}
(Fellow, IEEE) received the BS degree in electrical engineering from the National Taiwan University, and the MS and PhD degrees in electrical engineering from Stanford University in 1978. He is a distinguished professor with the University of Illinois at Chicago and Tsinghua University. He holds more than 300 US patents, is ACM fellow, is editor-in-chief of ACM Transactions on Knowledge Discovery from Data, and has been awarded several awards by IBM and the IEEE. His research interests are in the fields of data mining, social network, privacy preserving data publishing, data stream, database systems, and Internet applications and technologies. He is an ISI Highly Cited researcher. According to Google Scholar, his H-index is among the ten highest in computer science.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=0.9in,keepaspectratio,clip]{biophoto/shirui-bio.jpg}}]{Shirui Pan}
received a Ph.D. in computer science from the University of Technology Sydney (UTS), Ultimo, NSW, Australia. He is a Professor with the School of Information and Communication Technology, Griffith University, Australia. Prior to this, he was a Senior Lecturer with the Faculty of IT at Monash University. His research interests include data mining and machine learning. To date, Dr Pan has published over 200 research papers in top-tier journals and conferences, including TPAMI, TKDE, TNNLS, ICML, NeurIPS, and KDD.  His research received the 2024 CIS IEEE TNNLS Outstanding Paper Award and the 2020 IEEE ICDM Best Student Paper Award. He has been recognised as one of the AI 2000 AAAI/IJCAI Most Influential Scholars in Australia since 2021. He is an ARC Future Fellow and a Fellow of the Queensland Academy of Arts and Sciences (FQA). He is an Associate Editor of Neural Networks, Knowledge and Information Systems, IEEE Transactions on Cognitive and Developmental Systems, and IEEE Transactions on Cybernetics (TCYB).
\end{IEEEbiography}

\endgroup


